Planning with SiMBA: Motion Planning under Uncertainty for Temporal Goals using Simplified Belief Guides

This paper presents a new multi-layered algorithm for motion planning under motion and sensing uncertainties for Linear Temporal Logic specifications. We propose a technique to guide a sampling-based search tree in the combined task and belief space using trajectories from a simplified model of the system, to make the problem computationally tractable. Our method eliminates the need to construct fine and accurate finite abstractions. We prove correctness and probabilistic completeness of our algorithm, and illustrate the benefits of our approach on several case studies. Our results show that guidance with a simplified belief space model allows for significant speed-up in planning for complex specifications.

==> sections/Abstract.tex <==
\begin{abstract}
    This paper presents a new multi-layered algorithm for motion planning under motion and sensing uncertainties for Linear Temporal Logic specifications. We propose a technique to guide a sampling-based search tree in the combined task and belief space using trajectories from a simplified model of the system, to make the problem computationally tractable. Our method eliminates the need to construct fine and accurate finite abstractions. We prove correctness and probabilistic completeness of our algorithm, and illustrate the benefits of our approach on several case studies. Our results show that guidance with a simplified belief space model allows for significant speed-up in planning for complex specifications.
\end{abstract}

==> sections/Analysis.tex <==
\section{Theoretical Guarantees}
\label{sec:analysis}
In the following, we analyze the theoretical guarantees of our proposed framework.
% \qh{Check this assumption for $\neg O$ type of problems}

\begin{theorem}[Correctness]
    \label{theorem:correctness}
    Let $\text{V}^* = (\text{v}_0, \cdots, \text{v}_f)$ be a returned solution trajectory from the belief search layer. Then, the generated word of its continuous component is guaranteed to satisfy $\phi$, i.e., $\sigma \models \phi$.
\end{theorem}
\begin{proof}[Proof Sketch]
    $\text{V}^*$ is only returned as a solution if $\text{v}_f.q \in F$. Given polytopic regions $\mathcal{P}$, the computation of chance constraints for labels in \eqref{eq:belief integral} is conservative. Since the belief covariance $(\Sigma$ + $\Lambda)$ is computed exactly, the label is conservatively computed, i.e., $L(b_k)$ is correct. Thus, the belief components of $\text{V}^*$ (belief trajectory $\mathbf{b}$) correctly returns an accepting run on $\automaton$, so $\mathbf{b}$ satisfies $\phi$, i.e., $\mathbf{b} \models \phi$.
\end{proof}

% \begin{proof}[Proof Sketch]
%     A tree node is valid if its label causes a transition that is valid in the automaton. Given polytopic regions $\mathcal{P}$, the computation of chance constraints for labels in \eqref{eq:belief integral} is conservative. Since the belief covariance $(\Sigma$ + $\Lambda)$ is computed exactly (with no additional assumptions on the measurements obtained), the label $L(b_k)$ is conservatively computed, i.e., $L(b_k)$ is correct. $V^*$ is only returned as a solution if $v_f.q \in F$. The belief components of $V^*$ (belief trajectory $\mathbf{b}$) returns an accepting run on $\automaton$, which accepts precisely the traces that satisfies $\phi$, i.e., $\mathbf{b} \models \phi$.
% \end{proof}

% Let $T = (V, U)$ be the tree obtained from the algorithm for some iterations $N \in \mathbb{N}$. 

%Additionally, observe that the covariance $(\Sigma$ + $\Lambda)$ provides the distribution over possible covariances. 

% \begin{corollary}
%     Given a returned solution tree trajectory $V^* = (v_0, \cdots, v_T)$, the generated word of its continuous component is guaranteed to satisfy $\phi$, i.e., $\sigma \models \phi$.
% \end{corollary}

% with its associated controller $U^* = (u_0, \cdots, u_{t-1})$

\begin{theorem}[Probabilistic Completeness]
    Given an admissible \sbd, our framework is probabilistically complete.
\end{theorem}
%, i.e., it finds a solution if one exists almost surely as time approaches infinity.
% This is independent of the choice of SiMBA.

\begin{proof}[Proof Sketch]
    This follows from Theorem~\ref{theorem:correctness}, the definitions of admissible \sbd, and the results of \cite{Ho2022}.  Since automaton edge weights are updated at each iteration, every accepting run in $\automaton$ will be sampled infinitely often in the limit. In the limit, the search space will be covered by infinitely dense trees for both \sbd guide and belief search layers, following the probabilistic completeness of GBT. From Theorem~\ref{theorem:correctness}, any returned solution is guaranteed to be correct. 
\end{proof}

% \begin{proof}[Proof Sketch]
%     This follows from \ref{theorem:correctness}, the definitions of admissible \sbd, and the results of \cite{Ho2022}.  Since automaton edge weights are updated at each iteration, every accepting run in $\automaton$ will be sampled infinitely often in the limit. For each accepting run, the search space will be covered by infinitely dense trees for both \sbd guide and belief search layers, following the probabilistic completeness of GBT. In the limit, there will be an infinitely dense hybrid tree in the search space of Problem~\ref{prob:1}.  From Theorem~\ref{theorem:correctness}, any solution output for this tree is guaranteed to be correct. 
% \end{proof}

Note that we can always ensure probabilistic completeness even with an inadmissible \sbd.  This can be achieved by giving a separate time bound to the \sbd layer and conducting belief search without any \sbd guide if no solution is found by the \sbd layer. However, guides from an admissible \sbd can greatly reduce computation time as seen in our evaluation.

% \qh{TODO: Two versions of the algorithm are discussed, one with admissible \sbd}

% \begin{theorem}[Asymptotic Near-Optimality]
%     \qh{I really want to talk about optimality, which I think it is, but our implementation does not currently have benchmarks for them... :(}
%     Suppose that an asymptotically optimal belief tree search planner is used for \qh{continuous motion planning}, then our framework is asymptotically optimal.
% \end{theorem}

==> sections/Conclusion.tex <==
\section{Conclusion and Future Work}

We presented a modular framework for motion planning with complex tasks for systems under both motion and measurement uncertainty. We showed that simplified belief models provide important information for guiding motion tree search for planning in belief space. Our proposed framework is correct by construction and probabilistically complete. Empirical evaluations demonstrate the efficiency and efficacy of the planner. Future work aims at analyzing how to design accurate simplified models for better guides.

% , and extending this framework to work with general nonlinear systems. 
% Belief abstraction methods

% Maybe combination of different simbas? Maybe keep previous iteration simbas?

% Possible to look at better ways to do belief abstraction methods.

==> sections/Experiments.tex <==
\section{Evaluations}
We demonstrate the effectiveness of our proposed framework, through benchmarks and illustrative case studies. 
% We first illustrate the efficiency of our approach in comparison benchmarks. Then, we demonstrate the algorithm in a simulated drone delivery scenario.

\begin{table*}[ht!]
    \centering
    %  The success rate is the number of solutions computed within the time limit, and the mean time and standard error are reported. For unsuccessful runs, we use the time limit $120s$ as the time taken.
    \caption{\small Benchmarking results for underwater inspection scenario. We report the mean time to solution and standard error of the mean. Unsuccessful runs are given the maximum time of $120s$.
    % The scores within $10\%$ of the best scores for each specification are bold.\zs{Can we add uncertainty quantification for the \% successful?}
    The best scores are shown in bold fond. 
    }
    \label{tab:benchmarking}
    \scalebox{0.93}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{Algorithm} & \multicolumn{2}{c|}{$\phi_1$} & \multicolumn{2}{c|}{$\phi_2$} & \multicolumn{2}{c|}{$\phi_3$} & \multicolumn{2}{c|}{$\phi_4$} & \multicolumn{2}{c}{$\phi_5$}\\
    % \hline
    & Succ. (\%) & Time (s) & Succ. (\%) & Time (s) & Succ. (\%) & Time (s) & Succ. (\%) & Time (s) & Succ. (\%) & Time (s)\\\hline
    Abs-based& $0$ & NA & $0$ & NA & $0$ & NA & $0$ & NA & $0$ & NA\\
    Simba-free& $\mathbf{100}$ & $7.7 \pm 0.8$ & $66$ & $71.6 \pm 4.3$ & $63$ &  $78.7 \pm 4.0$ & $14$ & $114.1 \pm 1.7$ & $4$ & $117.7 \pm 1.2$\\
    Geo-\sbd& $\mathbf{100}$ & $6.9 \pm 0.6$ &  $89$ & $42.9 \pm 3.6$ & $81$ &  $59.3 \pm 4.2$ & $39$ & $103.5 \pm 2.6$ & $32$ & $107.3 \pm 2.4$\\
    SBA-\sbd& $\mathbf{100}$ & $\mathbf{5.8 \pm 0.5}$ & $\mathbf{95}$ & $\mathbf{29.3 \pm 2.9}$  & $\mathbf{92}$ &  $\mathbf{34.9 \pm 3.2}$ & $\mathbf{73}$ & $\mathbf{85.4 \pm 3.0}$ & $\mathbf{54}$ & $\mathbf{94.5 \pm 3.1}$\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
\end{table*}
\subsection{Simulation Benchmarks}

We compare our proposed framework with (i) a state-abstraction based approach (Abs-based), similar to extending \cite{Maly2013} to the belief space by using a belief space planner, and (ii) using our framework but without a \sbd layer as an ablation study, and using the full framework with different \sbds, (iii) a geometric \sbd that plans directly in the state space (Geo-\sbd), and (iv) SBA-\sbd which includes belief approximation as discussed in Sec.~\ref{sec:simba}.

% 

The scenario is a simplified underwater cave inspection with obstacles as depicted in Figure~\ref{fig:environment1}. Here, the robot can receive measurements with small noise about its state near the surface (in white), while it has to rely on noisier IMU otherwise. The robot has dynamics given by $\dot{x} = v \cos{(\theta)}, \dot{y} = v \sin{(\theta)}, \dot{\theta} = \omega, \dot{v} = a$.
% \begin{align*}
%     \dot{x} = v \cos{(\phi)}, \quad
%     \dot{y} = v \sin{(\phi)}, \quad \dot{\phi} = \omega,  \quad \dot{v} = a\text{,}
% \end{align*}
% with control input $u = (\omega, a)^T$. 
We use state feedback linearization to obtain a linearized closed loop model as in \cite{pairet2021, unicycle}. We consider the following increasingly complex LTLf formulas, with $a = \pi^{0.95}_a$ for region \textsc{a} (in green), $b = \pi^{0.95}_b$ for region \textsc{b} (in yellow), $c = \pi^{0.95}_c$ for region \textsc{c} (in white), and $o = \tilde{\pi}^{0.95}_o$ for region \textsc{o} (brown and black obstacles): 

% $\phi_1 = \globally \neg o \wedge \eventually a$, 
% $\phi_2 = \globally \neg o \wedge \eventually(a \wedge \eventually c)$, 
% $\phi_3 = \globally \neg o \wedge \eventually(a \wedge \eventually c) \wedge \eventually(b \wedge \eventually c)$, 
% $\phi_4 = \globally \neg o \wedge \eventually(a \wedge \eventually(c \wedge \eventually(a \wedge \eventually c)$, 
% $\phi_5 = \globally \neg o \wedge \eventually\big(a \wedge \eventually (c \wedge \phi_3)\big) \wedge \eventually\big(b \wedge \eventually (c \wedge \phi_3)\big)$. %\eventually(\phi_2 \wedge \tempop{X} \phi_2)$ \qh{This is written incorrectly}

\begin{itemize}
    \item $\phi_1 = \globally \neg o \wedge \eventually a$
    \item $\phi_2 = \globally \neg o \wedge \eventually(a \wedge \eventually c)$
    \item $\phi_3 = \globally \neg o \wedge \eventually(a \wedge \eventually c) \wedge \eventually(b \wedge \eventually c)$
    \item $\phi_4 = \globally \neg o \wedge \eventually(a \wedge \eventually(c \wedge \eventually(a \wedge \eventually c)$
    \item $\phi_5 = \globally \neg o \wedge \eventually\big(a \wedge \eventually (c \wedge \phi_3)\big) \wedge \eventually\big(b \wedge \eventually (c \wedge \phi_3)\big)$ %\eventually(\phi_2 \wedge \tempop{X} \phi_2)$ \qh{This is written incorrectly}
    
\end{itemize}

For each specification, $\globally \neg o$ refers to obstacle avoidance.
$\phi_1$ is a single goal motion planning problem, with the goal of reaching region $a$.
$\phi_2$ is a sequential goal problem, with the goal of reaching region $a$ followed by region $c$.
$\phi_3$ states that the robot should visit regions $a$ and $b$ in any order, before surfacing to region $c$.
$\phi_4$ states that the robot should visit regions $a$ followed by $c$ twice.
$\phi_5$ states that the robot should satisfy $\phi_3$ twice sequentially.

For belief tree planning, we used \cite{Ho2022} with RRT. We provided a time limit of $120s$ to find a solution for 100 trials. The results are summarized in Table~\ref{tab:benchmarking}. From the benchmarking results, it is evident that the state-abstraction approach does not work for belief space problems. This is due to the need to capture measurements affecting the belief dynamics in the abstraction. Note that it may be possible to combine abstraction-based approaches with a biased sampling paradigm, but it is not clear how to do so effectively. We also attempted to use belief discretization instead of state discretization, but it also performed poorly since many transitions in the abstraction are impossible.

Our results show that as complexity of specifications increases, so does the benefit of our planning scheme and the importance of \sbd guides. Even for reach-avoid task $\phi_1$, our planning scheme with both types of \sbds show better performance compared to the other methods, demonstrating the general efficacy of this approach for belief space planning with LTLf specifications. Furthermore, the addition of belief approximation in \sbd allows for more informative guides that reason about the belief space, leading to better solution times for SBA-\sbd as compared to Geo-\sbd. Typical solution trajectories returned by our proposed algorithm are shown in Figure~\ref{fig:environment1}, where the robot intelligently navigates close to the surface to localize (reduce uncertainty) before submerging and completing its tasks in the cave, through which measurements have higher noise values.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{}
%     \caption{Sea Example Environment}
%     \label{fig:sea_example}
% \end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
            \centering
            \includegraphics[width=\linewidth, , trim={7cm 2.5cm 6cm 2cm},clip]{figures/environment1_phi1_annotated.pdf}
            % \caption[$\phi_1$.]{$\phi_1$}
            % % {{\footnotesize }}    
            % \label{fig:phi1}
        \end{subfigure}
        \begin{subfigure}[b]{0.23\textwidth}  
            \centering 
            \includegraphics[width=\linewidth, trim={7cm 2.5cm 6cm 2cm},clip]{figures/environment1_phi2_annotated.pdf}
            % \caption[$\phi_2$.]%
            % {$\phi_2$}
        \end{subfigure}
        \caption[Effect of varying $p_{bias}$ on solution length with 10 seconds of planning time.]
        {\small Underwater inspection Scenario. $\phi_1$ (left): The robot moves close to the surface to localize before completing the task. $\phi_2$ (right): The robot completes sub-task $\eventually a$ (red trajectory) and nested sub-task $\eventually c$ (black trajectory).}  
            \label{fig:environment1}
        \vspace{-3mm}
\end{figure}

% \begin{subfigure}[b]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment1.pdf}
%         \caption[Environment 1.]%
%         {{\footnotesize Sea Cave Exploration}}    
%         \label{fig:sea example}
% \end{subfigure}

\begin{figure}[ht]
    \centering
     \begin{subfigure}[b]{0.22\textwidth}  
            \centering 
            \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment2_trajectory_topdown_annotated.pdf}
            % \caption[$\phi_2$.]%
            % {{\footnotesize Top Down View}}    
            % \label{fig:drone example}
        \end{subfigure}
        \begin{subfigure}[b]{0.23\textwidth}  
            \centering 
            \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment2_trajectory_side.pdf}
            % \caption[$\phi_2$.]%
            % {{\footnotesize Side View}}    
            % \label{fig:drone example}
        \end{subfigure}
        \caption[Environments. ]
        {\small Drone delivery, top down (left) and side (right) views.
        }
        \label{fig:environment2}
        \vspace{-5mm}
\end{figure}


%  \begin{subfigure}[b]{0.23\textwidth}  
%             \centering 
%             \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment2_trajectory_topdown_.pdf}
%             \caption[$\phi_2$.]%
%             {{\footnotesize Drone Delivery (top down).}}    
%             \label{fig:drone example}
%         \end{subfigure}
        
        
% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth}
%             \centering
%             \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment1.pdf}
%             \caption[Environment 1.]%
%             {{\footnotesize Sea Cave Exploration}}    
%             \label{fig:sea example}
%         \end{subfigure}
%         \begin{subfigure}[b]{0.23\textwidth}  
%             \centering 
%             \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment2_trajectory_topdown_.pdf}
%             \caption[$\phi_2$.]%
%             {{\footnotesize Drone Delivery (top down).}}    
%             \label{fig:drone example}
%         \end{subfigure}
%         \caption[Environments. ]
%         {\small Environments
%         }
%         % \label{fig:solutionpaths}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth}
%             \centering
%             \includegraphics[width=\linewidth, , trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment1_phi1.pdf}
%             \caption[$\phi_1$.]%
%             {{\footnotesize $\phi_1$: The robot navigates close to the surface to localize before navigating to region $a$.}}    
%             \label{fig:phi1}
%         \end{subfigure}
%         \begin{subfigure}[b]{0.23\textwidth}  
%             \centering 
%             \includegraphics[width=\linewidth, trim={7cm 2.5cm 7cm 2cm},clip]{figures/environment1_phi2.pdf}
%             \caption[$\phi_2$.]%
%             {{\footnotesize $\phi_2$: The robot completes sub-task $\eventually a$ (black trajectory) and nested sub-task $\eventually c$ (red trajectory).}}    
%             \label{fig:phi2}
%         \end{subfigure}
%         \caption[Effect of varying $p_{bias}$ on solution length with 10 seconds of planning time.]
%         {\small Sea Cave Inspection Environment.
%         }
%         \label{fig:sea solutionpaths}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.7\linewidth, , trim={7cm 2.5cm 5cm 2cm},clip]{figures/environment2_trajectory_side.pdf}
%     \caption{\small Drone delivery problem in $\phi_6$, with $95\%$ covariance ellipses.}
%     \label{fig:drone solutionpaths}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth}
%             \centering
%             \includegraphics[height=3.5cm, width=\linewidth]{figures/environment2_trajectory.png}
%             \caption[$\phi_6$ side view.]%
%             {{\footnotesize Side View.}}    
%             \label{fig:phi6}
%         \end{subfigure}
%         \begin{subfigure}[b]{0.23\textwidth}
%             \centering 
%             \includegraphics[height=3.5cm, width=\linewidth]{figures/environment2_trajectory_topdown.png}
%             \caption[$\phi_6$. top down view]%
%             {{\footnotesize $\phi_7$ top down view.}}    
%             \label{fig:phi6_topdown}
%         \end{subfigure}
%         \caption[]
%         {\small Drone delivery problem, with $95\%$ covariance ellipses.
%         }
%         \label{fig:drone solutionpaths}
% \end{figure}

% \begin{table}
%     \centering
%     \caption{Benchmarking results for $\phi_1$, with a 60 second time limit, $Q = 0.1$ The success rate is the number of solutions computed within the time limit, and the mean time to first solution and standard deviation are reported. \qh{Needs update}}
%     \label{tab:benchmarking}
%     \scalebox{0.96}{
%     \begin{tabular}{l|c|c|c|c}
%      & \multicolumn{2}{c|}{2D Problem} & \multicolumn{2}{c}{3D Problem}\\
%     % \hline
%     Algorithm &  Succ. (\%) & Time (s) & Succ. (\%) & Time (s)\\\hline
%     Syclops-GBT& $\mathbf{??}$ & $\mathbf{?? \pm ??}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     Naive-GBT& $\mathbf{100}$ & $6.32 \pm 0.89$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     GeoSiMBA-GBT& $\mathbf{100}$ & $\mathbf{5.02 \pm 0.36}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     FullSiMBA-GBT& $\mathbf{100}$ & $\mathbf{4.89 \pm 0.41}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$
%     \end{tabular}
%     }
% \end{table}

% \begin{table}
%     \centering
%     \caption{Benchmarking results for $\phi_1$, with a 60 second time limit, $Q = 0.15$ The success rate is the number of solutions computed within the time limit, and the mean time to first solution and standard deviation are reported. \qh{Needs update}}
%     \label{tab:benchmarking}
%     \scalebox{0.96}{
%     \begin{tabular}{l|c|c|c|c}
%      & \multicolumn{2}{c|}{2D Problem} & \multicolumn{2}{c}{3D Problem}\\
%     % \hline
%     Algorithm &  Succ. (\%) & Time (s) & Succ. (\%) & Time (s)\\\hline
%     Syclops-GBT& $\mathbf{??}$ & $\mathbf{?? \pm ??}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     Naive-GBT& $96$ & $21.66 \pm 2.19$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     GeoSiMBA-GBT& $\mathbf{100}$ & $17.74 \pm 1.8$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     FullSiMBA-GBT& $\mathbf{100}$ & $\mathbf{14.96 \pm 1.56}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$
%     \end{tabular}
%     }
% \end{table}

% \begin{table}
%     \centering
%     \caption{Benchmarking results for $\phi_2$, with a 60 second time limit, $Q = 0.2$ The success rate is the number of solutions computed within the time limit, and the mean time to first solution and standard deviation are reported. \qh{Needs update}}
%     \label{tab:benchmarking}
%     \scalebox{0.96}{
%     \begin{tabular}{l|c|c|c|c}
%      & \multicolumn{2}{c|}{2D Problem} & \multicolumn{2}{c}{3D Problem}\\
%     % \hline
%     Algorithm &  Succ. (\%) & Time (s) & Succ. (\%) & Time (s)\\\hline
%     Syclops-GBT& $\mathbf{??}$ & $\mathbf{?? \pm ??}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     Naive-GBT& $96$ & $14.14 \pm 1.97$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     GeoSiMBA-GBT& $\mathbf{96}$ & $12.84 \pm 2.06$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$\\
%     FullSiMBA-GBT& $\mathbf{98}$ & $\mathbf{8.07 \pm 1.31}$ & $\mathbf{??}$ &  $\mathbf{?? \pm ??}$
%     \end{tabular}
%     }
% \end{table}

\subsection{Urban Drone Delivery}

Next, we demonstrate our algorithm in a simulated drone delivery problem in an urban environment, as depicted in Figure~\ref{fig:environment2}.
% \qh{Can remove this equations and link to Eric's paper if space constrained}
% \begin{align*}
%     \dot{x} = v \cos{(\phi)}\cos{(\theta)}, \quad
%     \dot{y} = v \sin{(\phi)}\cos{(\theta)}, \\
%     \dot{z} = v\sin{(\theta)}, \quad \dot{\phi} = \omega,  \quad \dot{\theta} = q\text{.}
% \end{align*}
% with control input $u = (v, \omega, q)^T$. The Gaussian process describing the UAV's motion model is learnt from data following \cite{pairet2021}. 
Details on the dynamics can be found in Appendix~A.2 of \cite{pairet2021}.
We consider a delivery problem, where UAV has to pick up a package at the foot of a building A (region \textsc{a} in blue), and deliver it to foot of building B (region \textsc{b} in yellow) while avoiding obstacles (in gray). Additionally, it can only receive GPS measurements if it flies above the gray buildings (in light green), but it cannot fly that high after picking up a package. In LTLf, this task is $\phi_6 = \globally \neg o \wedge \eventually(a \wedge \eventually b) \wedge \globally (a \implies \globally \neg c)$, with $a = \pi^{0.99}_a$, $b = \pi^{0.99}_b$, $c= \tilde{\pi}^{0.99}_c$, and $o= \tilde{\pi}^{0.99}_{o}$. We conducted $100$ trials for this problem with time limit of $120s$, and our algorithm with SBA-\sbd found a solution with $90\%$ success rate, with mean time to solution of $30 \pm 4.1$. A typical solution is shown Figure~\ref{fig:environment2}. The UAV first flies above the buildings as an information gathering action to reduce its uncertainty, before flying to region \textsc{a} and then \textsc{b}, to ensure that its uncertainty is low enough to reach both regions with high probability.

==> sections/Introduction.tex <==
\section{Introduction}

% \ml{\\
% P1: realistic robots have both motion and sensor uncertainty... robotic tasks are complex... motion planning with both uncertainties is hard... this paper focuses on this challenge\\ \\
% P2: LTL is used to express complex tasks... most work focus on motion uncertainty, and abstract to MDP with objective of maximizing the probability of success.  Some recent work focus on both uncertainties and abstract to POMDP. LTL synthesis on POMDPs is hard/expensive, not scalable.\\ \\
% P3: Recent work in motion planning under uncertainty use the power of sampling-based techniques and combine it with chance constraint.  This is a relaxation of maximizing probability of success.  The results is a plan as a sequence of controls, instead of a policy.  Most work focus on motion uncertainty.  Recent work also include sensor uncertainty.  They are however limited to A-to-B planning. \\ \\
% P4: What this work does...\\ \\
% P5: Contributions!
% }

% As robots become more advanced, robotic tasks have also increased in complexity.  The ability for robots to efficiently synthesize complex behaviors is thus an essential challenge. 
As robots become more advanced, the expectation for them to perform tasks with higher complexities increases. 
It is thus an essential challenge to enable efficient planning for complex requirements. In addition, real-world robots must be able to reason about both motion and sensor uncertainty while executing such tasks. For instance, an autonomous underwater rover often has noisy motion due to water currents and gets accurate GPS measurements only at the surface; under the surface sensor readings are highly noisy. The combination of accounting for these uncertainties with the need to provide guarantees for task completion makes the planning problem very difficult. This paper focuses on this challenge and aims to develop an efficient framework for planning under uncertainty with complex specifications.

Linear Temporal Logic (LTL) is a principled formalism for expressing complex temporal tasks for robotic systems \cite{ltlf, Hadas2018Review, Fainekos2005}. For instance, a robot tasked with ``visit A and B in any order, and then go to C while avoiding D" can be expressed precisely as an LTL formula. The primary existing LTL motion planning frameworks for continuous state and action spaces are designed for deterministic systems \cite{Bhatia2010, Maly2013, Luo2021, Plaku2016}.
% In this work, we use LTL to specify our tasks for systems under uncertainty.

To address LTL synthesis problems for systems with uncertainty, works \cite{Wells2020, Ding2012, Luna:WAFR:2015} focus solely on motion uncertainty.  They first abstract the evolution of the robot in the environment into a finite Markov Decision Process (MDP), and then synthesize a policy that maximizes the probability of successfully completing the LTL specification. For observation uncertainty, LTL synthesis on Partially Observable MDPs have recently been proposed for moderately-sized discrete space problems \cite{Bouton2020}, or through finite state abstraction of continuous spaces \cite{haesaert2018}. However, a common limitation of these works is the need for a finite abstraction from continuous states and actions to discrete ones. There are currently no methods that can give practically useful guarantees for general continuous-space POMDPs.

% Optimization-based methods have also been employed to synthesize controllers for temporal logic specifications for systems under uncertainty \cite{jha2018safe, Sadigh2016RSS}. However, these methods are not fully applicable to many robotics problems since they require a fixed horizon, and the horizon for motion planning problems is usually unbounded. These approaches thus suffer with scalability issues or do not provide task completion guarantees for temporal planning problems that require long horizons. \ml{this paragraph is vague}

% By using a fixed receding horizon approach, one loses guarantees on task completion for motion planning and suffers with scalability for longer horizon problems.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,  trim={2.5cm 4cm 3.5cm 4cm},clip]{figures/ICRA23.pdf}
    \caption{Planning with SiMBA Framework}
    \label{fig:overview}
    \vspace{-6mm}
\end{figure}

For continuous spaces, recent works in motion planning under uncertainty combine the power of sampling-based methods \cite{Kingston2018} with point-wise chance-constraints on the probability of safety \cite{cc-rrt, blackmore2011, cc-rrt*, firm, bry2011rrbt, Ho2022, Zheng2022}. This is a relaxation of maximizing success probability, but it allows for fast and scalable motion planning with robustness guarantees. Most works focus on motion uncertainty \cite{blackmore2011, pairet2021, cc-rrt}, but recent works \cite{bry2011rrbt, Ho2022, firm, Zheng2022} introduce extensions to account for sensor uncertainty. While they provide efficient planning under uncertainty, they are limited to simple task of A-to-B planning. Recent work \cite{Oh2021} extends chance constrained planning to LTL tasks and minimizes the probability of task failure, but their approach is limited to systems under motion uncertainty.
% \ml{improper treatment of the task satisfaction?}

A main challenge in dealing with both uncertainty and complex specifications is the need to simultaneously account for both the belief and task spaces. Doing so results in extremely large search spaces. Principled guidance of a low-level motion tree has been shown to improve tractability in the deterministic setting for both single and multi-temporal goals planning, using layers of planning \cite{Plaku2010syclops, Maly2013, Ho2022CDC, Bhatia2010} or heuristic guidance \cite{Luo2021}. For stochastic systems, \cite{Tajvar2020} proposes a heuristic to guide tree extension, but their framework is only designed for dynamics noise. Extending these techniques to settings with both motion and measurement uncertainty is non-trivial because of the difficulty in constructing a guidance mechanism that captures belief dynamics well.

In this paper, we present a multi-layered framework to synthesize motion plans for LTL tasks for systems under both motion and measurement uncertainty. The LTL tasks are defined in the belief space with a user-defined robustness requirement. We show that our framework provides guarantees on task completion and probabilistic completeness. 

Our approach has two novel characteristics: First, we introduce a method to plan over an automaton that represents the LTL task directly that avoids the need for fine abstraction, by pruning infeasible edges. Second, in order to make the problem computationally tractable, we propose to use a simplified model that accounts for both motion and measurement uncertainty. We refer to this notion as Simplified Models with Belief Approximation (\sbd), which we use to rapidly find a continuous path that heuristically guides the search for a satisfying motion plan for the full system. Our evaluation shows that the addition of \sbd for guidance improves solution time significantly. To the best of our knowledge, this is the first work that uses trajectories from a simplified model in the belief space to bias sampling-based search for stochastic systems under complex tasks.

In summary, the contributions of this paper are five-fold: (i) a framework for planning under LTL specifications for continuous systems under motion and measurement uncertainty with (ii) guarantees on task completion and probabilistic completeness; (iii) planning over a pruned automaton that alleviates the state explosion problem in abstraction-based methods; (iv) increasing efficiency by using a simplified model in the belief space to provide continuous trajectory guides for belief planning, and (5) a series of illustrative case studies and benchmarks.
% \zs{Low Priority: These are all different \emph{types} of contribution - perhaps we could make the story clearer to readers with a bit more structure, e.g. "We propose a framework for planning under ... with two novel characteristics: (a) [SiMBA] (b) [pruned automaton]. We show that this framework achieves [guarantees] and demonstrate with illustrative case studies and benchmarks." (the square brackets are places where we'd need to work out the wording.)}

% In this work, we also use biasing towards potential solutions in the task space by using a reduced order belief model of the system. Instead of geometric planning, we use a reduced-order belief model in order to capture the belief topology of the problem manifold for LTL specifications.

% We take advantage of the observation that lead paths that include a coarse belief representation are more informative guides than ones that do not.

% Effective balance between fast inaccurate plans and accurate plans.

% Contributions



==> sections/Methodology.tex <==
\section{Belief Space Planning with Simplified Belief Approximations}
\label{sec:beliefplanning}

We present a modular framework to solve Problem~\ref{prob:1}. The framework is inspired by \cite{Plaku2010syclops, Maly2013, pairet2021} and consists of three main layers: task planning layer, \sbd guide layer, and belief search layer, as depicted in Fig. \ref{fig:overview}.

% At the task planning layer, we first translate the LTLf formula into an automaton. 
We first translate the LTLf formula $\phi$ into a Deterministic Finite Automaton (DFA). Then, we prune unrealizable transitions of the DFA, and use the pruned DFA for task planning. At each iteration, on the automaton, we find the shortest path that corresponds to a $\phi$-satisfying trace to use as a task plan. Then, at the \sbd guide layer, we use a simplified model of the system to rapidly find a path annotated with DFA states that obeys the task plan. We call this technique Simplified Models with Belief Approximation (\sbd). Finally, at the belief search layer, a sampling-based belief tree searches for a satisfying trajectory by using the full system. The growth of this tree is biased to search around the hybrid annotated path while still ensuring the motion plan satisfies $\phi$.

% \begin{algorithm}
%     \caption{Belief Space Planning for LTLf}
%     \label{alg:framework}
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \Input{$\phi, \tilde{X}$}
%     \Output{Motion Plan satisfying $\phi$}
%     $\mathcal{A} \leftarrow$ ConstructAutomaton$(\phi)$\\
%     $\automaton \leftarrow$ PruneAutomaton$(A, \mathcal{P})$ \\
%     \While{Time Elapsed $< t_{max}$}
%     {
%         $\taskplan \leftarrow \{(d_i, q_i)\}_{i \geq 0} \leftarrow$ TaskPlanner($\mathcal{P}, t_{max}$)\\
%         $\xi_{\tilde{X}} \leftarrow \sbd()$\\
%         $(\mathbf{v}, \mathbf{u}, \taskplan) \leftarrow$ Explore($\taskplan, \textsc{tr}, \mathcal{P}, X, t_{e}$)\\
%         \If{$(\mathbf{v}, \mathbf{u}, \taskplan) \neq \emptyset$}{
%             \Return $(\mathbf{v}, \mathbf{u}, \taskplan)$
%         }
%     }
%     \Return No Solution
% \end{algorithm}

\subsection{Belief Propagation and Labeling}
\label{sec:beliefpropagationandlabel}
% \ml{isn't this subsection all from CC-RRT paper? Why do we repeat it? Maybe present the ideas at the high-level and refer the reader to the paper for the detials and equations?}
% \qh{Yes,  eq. (13)-(16) are in Blackmore's paper, but I think we should have the equations in this paper because these equations are not explicitly written in the original paper (stay-in regions, not obstacle regions). I think it'd be helpful for readers to see the equations in this paper to see how labelling can be done for polytopic obstacles, or we could also put them in the preliminaries.}

% \ml{maybe change the subsection title to Belief propagation and labeling, move the belief propagation equations here, and briefly talk about how the labels can be generated for each belief.}

Here, we establish the relationship between the evolution of the distribution over robot state, atomic predicates, and labels.
During offline planning, following \cite{bry2011rrbt, Ho2022}, given a stabilizing feedback controller in \eqref{eq:feedback controller} and online state estimate $\xhat_k$, 
% \begin{align}
%     x_k = Ax_k + B(\check{u}_{k-1} - K(\hat{x}_k - \check{x}_k)) + w_k\text{.}
% \end{align}
We parameterize the belief at each time step based on the closed loop dynamics as:
\begin{align}
    \label{eq:belief}
    x_k \sim b_k = \N(\checkx_k, \cov^+ + \Lambda_k^+ ),
\end{align}
where $\cov^+$ is the covariance that represents the online state estimation error, and $\Lambda_k^+$ is the covariance matrix of $\hat{x}_k$, which is a random variable when planning offline. It 
% represents the uncertainty over possible state estimates that could arise during online execution of the motion plan and is a result of considering all possible measurements received.
accounts for the uncertainty related to the measurements when executed online.
Analogous to the Kalman Filter, covariance matrices $\cov^+$ and $\Lambda_k^+$ can be computed recursively:
\begin{align}
    \label{eq:belief_propagation_equations}
    \cov^- &= A\Sigma_{k-1}^+A^T + Q,\\
    L_k &= \cov^-C^T(C\cov^-C^T + R(\xhat_k))^{-1},\\
    \cov^+ &= \cov^- - L_kC\cov^-,\\
    \Lambda_k^+ &= (A- BK)\Lambda_{k-1}^+(A-BK)^T + L_kC\cov^- \text{.}\label{eq:beliefpropagation}
\end{align}

Given belief $b_k$, its label $L(b_k)$ is the set of atomic propositions in $\Pi$ that are true in $b_k$, i.e., $\pi_i^{\alpha_i} \in L(b_k) \iff P(x_k \in p_i) > 1 - \alpha,$ where
\begin{align}
    \label{eq:belief integral}
    P(x_k \in p_i) = \int_{p_i} \N(s \mid \checkx_k, \cov^+ + \Lambda_k^+ ) ds.
\end{align}

Since our regions are convex polytopes that can be described as a conjunction of linear half-spaces, we can 
% provably conservatively 
efficiently compute bounds for \eqref{eq:belief integral}, using methods such as those described in \cite{blackmore2011, cc-rrt, Liu2014, pairet2021}.

% We use the following proposition to compute the label:
% \qh{TODO: Remove this proposition and add methods to compute $L(b_k)$}
% \ml{Need a transition sentence to the proposition if you decide to keep it}
% \begin{proposition}
%     Given $b_k = \N(\check{x}_k, (\Sigma_k + \Lambda_k)$, convex polytopic region $p_i$ described as a conjunction of linear half-spaces, probability bound $\alpha$, and following \cite{blackmore2011}, we can compute $L(b_k)$ using the following: 
%     \begin{align}
%          \bigwedge_{j \in p_i} (b_j - a_j^T \check{x}_k \geq c) \implies P(x_k \in p_i) \geq 1 - \alpha
%     \end{align}
%     where
%     \begin{align}
%         &c = \sqrt{2a_j^T (\Sigma_k + \Lambda_k) a_j} \cdot \mathrm{erf}^{-1}(1 - 2\delta),
%     \end{align}
%     where $\mathrm{erf}(\cdot)$ is the error function, such that $\sum_{j \in p_i}\delta \leq \alpha$.
% \end{proposition}

% We first note that $p_i \in \mathcal{P}$ is a convex polytopic region, hence, it can be described as a conjunction of a set of linear half-spaces (constraints) as follows:
% \begin{align}
%     x_k\in p_i \iff \bigwedge_{j \in p_i} a_j^T x_k \leq b_j,
% \end{align}

% Therefore, checking if \eqref{eq:belief integral} is less than $1-\alpha_i$ can be done by chance constraints over linear regions. For a given belief state $b_k$, linear chance constraints can be expressed exactly as deterministic linear constraints using the method discussed in \cite{blackmore2011}, as follows.

% For each linear constraint,
% \qh{Check this math}
% \begin{align}
%     \label{eq:exactconstraint}
%     P(a_i^T x_k \leq b_i) > 1 - \alpha \iff b_i - a_i^T \check{x}_k \geq c,
% \end{align}

% where
% \begin{align}
%     &c = \sqrt{2a^T (\Sigma_k + \Lambda_k) a} \cdot \mathrm{erf}^{-1}(1 - 2\alpha),
% \end{align}
% where $\mathrm{erf}(\cdot)$ is the error function.

% Using this transformation, we can compute labels for a belief. 

% \qh{Check whether this is wrong because we compute stay in and stay out regions differently.}

% We now consider the following assumptions. 
% \ml{why?}

% \qh{These assumptions are here as a placeholder, we should move them, but I don't know where}\zs{Do we actually need these assumptions mathematically, or are they just there to justify our search heuristics? (maybe I will find the answer by reading more)}\qh{We need these mainly assumptions to theoretically analyze a search heuristic model} 

% \begin{assumption}
%     \label{as:covariance decrease phi better}
%     If $b_a = \mathcal{N}(\check{x}, \Sigma_a)$, $b_b = \mathcal{N}(\check{x}, \Sigma_b)$, and $\Sigma_a < \Sigma_b$, then 
%     \begin{itemize}
%         \item For $\alpha < 0.5$: $\pi^{\alpha} \in L(b_b) \implies \pi^{\alpha} \in L(b_a)$.
%         \item For $\alpha > 0.5$: $\pi^{\alpha} \notin L(b_b) \implies \pi^{\alpha} \notin L(b_a)$
%     \end{itemize}
% \end{assumption}

% \;\forall \pi^{\alpha_i}_i \in \{\pi^{\alpha_i}_i \in \Pi \mid \alpha_i < 0.5\}
% \;\forall \pi^{\alpha_j}_j \in \{\pi^{\alpha_j}_j \in \Pi \mid \alpha_j > 0.5\}$
% \noindent Intuitively, this states that increasing the covariance does not increase the probability of being in a region at a given state mean for low $\alpha$, which corresponds to `reach' regions.

% % \begin{assumption}
% %     \label{as: covariance decrease CC better}
% %     If $b_a = \mathcal{N}(\check{x}, \Sigma_a)$, $b_b = \mathcal{N}(\check{x}, \Sigma_b)$, and $\Sigma_a < \Sigma_b$, then $\pi^{\alpha_j}_j \notin L(b_b) \implies \pi^{\alpha_j}_j \notin L(b_a)\;\forall \pi^{\alpha_j}_j \in \{\pi^{\alpha_j}_j \in \Pi \mid \alpha_j > 0.5\}$.
% % \end{assumption}
% \noindent Intuitively, this states that increasing the covariance does not increase the probability of not being in a region at a given state mean for high $\alpha$, which corresponds to 'avoid' regions.

% These assumptions may be violated for problems with very small regions and systems with high covariances, but is reasonable for many problems in robotics since we do not generally want to increase uncertainty in order to satisfy chance constraints. This assumption is not required for the correctness of our proposed framework, but we use this intuition to build our \sbd guiding methodology.
% , especially for LTLf formulas with $\alpha$ close to 0 or 1.

% \qh{Generalyl we don't need this, but generally we care about not adding uncertainty to satisfy stuff. We build our simba framework based on this intuition}

\subsection{Task Planning with Pruned Automaton}

At the task planning layer, an automaton is used to define a sequence of sub-tasks the robot has to complete.

\subsubsection{Automaton Construction and Pruning}

An LTLf formula $\phi$ can be translated into a minimized Deterministic Finite Automaton (DFA) 
% $\automaton$ 
that represents precisely the traces that satisfies $\phi$ \cite{ltlf}. 
% Thus, we first construct $\automaton$, the minimized DFA of the given LTLf formula $\phi$. 
A DFA is defined as a tuple $\automaton = (Q, q_0, S,  \delta, F)$, where $Q$ is a finite set of states, $q_0 \in Q$ is the initial states, $S= 2^\Pi$ is a set of input symbols, $\delta : Q \times S \rightarrow 2^Q$ is the transition function, $F \subseteq Q$ is the set of accepting states.

Instead of planning over a product automaton (cartesian product between $\automaton$ and a finite abstraction of the robotic system) like in \cite{Oh2021, Maly2013, Bhatia2010, Kantaros2020, Ho2022CDC}, we propose to use the abstraction to prune impossible task sequences of $\automaton$. To do this, we construct an adjacency graph of the regions in $\mathcal{P}$ in order to prune impossible transitions in $\automaton$. 

% \qh{Not sure what the best word is. Trivially is used because not all impossible transitions are removed, but just the ones that are geometrically impossible}\qh{eliminate abstraction usage}

The adjacency graph is constructed by computing adjacency and intersections between the regions in $\mathcal{P}$ as well as the remainder region $X \setminus \cup_{p \in \mathcal{P}}$. Each region is represented as a node in the adjacency graph, and edges of the graph represent regions which are geometrically adjacent to each other or intersecting with one another. 
% We also add an additional node connected to all other nodes, which represents the empty symbol. 
This adjacency graph captures the possible transitions between regions in the continuous state space, and we use it to remove geometrically impossible letters in the alphabet, thereby pruning the edges in $\automaton$ that are not realizable in the state space. 
% \ml{well ... not only that... the edges of the adjacency graph also help to remove infeasible edges of the DFA}
% \qh{That is what I'm trying to write here actually. Is that unclear?}

% \qh{Need to handle the case where one region subsumes another region, maybe?}
% \ml{no, if the intersection is defined as its own region/node, then, it's already taken care of.}\qh{I'm thinking of the edge between the added empty symbol node and the subsumed region}

This approach has two advantages. First, it removes the need for fine abstractions of the problem space and system, which improves scalability by alleviating the state explosion problem. Our approach generalizes the method proposed by \cite{Luo2021}, by providing a way to prune the automaton using information about $\mathcal{P}$. Second, our method allows the belief planners in the subsequent layers the freedom to explore the belief space without restrictions, which is important for belief space planning, especially when the measurement noise is state dependent as in our problem, i.e., $\mathcal{R}(x_k)$.

Task planning is directly performed on $\automaton$ by augmenting it with weights over edges that represent estimates on motion tree feasibility. These weights are continuously updated during the planning process.

\subsubsection{Task Planning}
In each iteration of task planning, 
% we search the pruned and weighted $\automaton$. By searching $\automaton$,  
we compute 
an accepting run (task plan) $\taskplan$ 
% is computed. 
on the pruned and weighted $\automaton$.
A graph search algorithm, such as $A^*$, is used to find the shortest path to an accepting state in $F$ from the initial state $q_0$. Each task plan is a candidate sequence of automaton states that the algorithm uses to lead 
% \qh{lead and guide are basically the same thing, but guides are already used for \sbd. How do we differentiate better?} 
% a sampling-based motion tree of belief trajectories in 
the search in the
subsequent layers. By finding a belief trajectory that follows $\taskplan$, the robot is guaranteed to satisfy 
% the LTLf specification 
$\phi$.

% \ml{the last statement is not quite true... the probability of being in the regions should be considered since the atomic propositions have $\alpha$ parameter.}\qh{The task plan is a sequence of automaton states, so the probability of being in a region is baked into the word generated because of $L(b_k)$, no?}

% \qh{ provide motivation for the weighting function}

To define the feasibility edge weights of $\automaton$, we first assign a weight to each state.
% For each automaton state $q \in Q$, we assign a weight defined by
For state state $q \in Q$,
\begin{align}
    \label{eq:automatonweights}
    w(q) = \frac{(cov(q) +1)}{DistFromAcc(q) \cdot (numsel(q) +1)^2},
\end{align}
where $cov(q)$ is the number of motion tree vertices associated with $q$, $numsel(q)$ is the number of times $q$ has been selected, and $DistFromAcc(q)$ is the shortest unweighted path from $q$ to an accepting state in $F$. $DistFromAcc(q)$ can be computed using an unweighted graph search algorithm such as Djikstra's Algorithm 
% \qh{DistFromAcc may not really make sense here since we are planning directly on the automaton, but my implementations are based on this so...}, 
and can be computed once beforehand. Then, the edge weight between states $q,q' \in Q$ is 
% defined as 
% \begin{align}
%     w(q,q') = (w(q)\cdot w(q'))^{-1}.
% \end{align}
$w(q,q') = (w(q)\cdot w(q'))^{-1}.$

% These weights are updated in every iteration of the belief search layer. 
This weighting scheme promotes search in unexplored parts of the task space and suppresses search in parts 
% of the task space 
where attempts at finding a solution have repeatedly failed.

\subsection{Hybrid Tree Search: Gaussian Belief Trees with DFAs}
\label{sec:gbt}
For belief space planning with both the simplified model and full constrained model, we use Gaussian Belief Trees (GBT) in \cite{Ho2022} as our base belief space planner in a hybrid discrete-continuous tree search planner. The hybrid planner is similar to the frameworks for deterministic LTL planners in \cite{Maly2013,Bhatia2010, Ho2022CDC}, but we plan directly with automaton states instead of product automaton states. Also, we reason about robot uncertainty while planning. For completeness of presentation, we provide a brief overview of this method.

Given a task plan $\taskplan$, we compute the set of DFA states $Q_T$ that exist in $\taskplan$ and contain at least one tree vertex at every iteration. The hybrid tree search expands in $Q_T$. In each iteration, a DFA state $q$ is sampled from $Q_T$. A tree vertex $\text{v}_s$ is sampled among vertices that have discrete components $q$, and one iteration of GBT is performed to obtain a new vertex $\text{v}_n$. A tree vertex is a tuple $\text{v} = (\check{x}, \Sigma, \Lambda, q)$. An iteration of GBT involves selecting a tree vertex $\text{v}_{sel}$, sampling a valid nominal control $\check{u} \in U$, and propagating the continuous belief components in $\text{v}_{sel}$ to obtain the new belief $(\check{x}_n, \Sigma_n, \Lambda_n)$, according to \eqref{eq:system} and Sec.~\ref{sec:belief_propagation_equations}. The new discrete state component $q_n$ of $text{v}_n$ is obtained by propagating the automaton with the label of the new belief.

% \zs{Probably too much to do before deadline: this might be easier to parse if it was a psuedocode algorithm.}

%with probability proportional to the weights in $Q$

Vertex $\text{v}_n$ is valid and added to the tree if both its continuous and discrete state components are valid. The continuous component $\text{v}_n.b = (\text{v}_n.\check{x}, \text{v}_n.\Sigma, \text{v}_n.\Lambda)$ is valid if it obeys the constraints of \eqref{eq:system}. The discrete component $\text{v}.q$ is valid if it exists in the DFA. Finally, if $\text{v}_n.q$ is an accepting state, the motion plan $(\check{U}, \check{X})$ and corresponding tree vertices $\mathbf{\text{v}}$ ending with $\text{v}_n$ is returned as a solution.

% Suppose that a new vertex $v_n$ corresponds to a newly reached automaton state that is in the current task plan $\taskplan$, this automaton state is added to $Q$ for exploration in the next iteratons. 

\subsection{\sbd Layer for LTLf Guides}
\label{sec:simba}
% \qh{Need a paragraph to link this guide to just using automaton, and not product automaton}

% \ml{should combine the next 2 paragraphs into one and make is succinct.}
Once a task plan is generated, we can directly use the hybrid tree search with Gaussian Belief Trees using System~\eqref{eq:system} to attempt to satisfy the task sequence constraints. However, a naive method of tree search is computationally inefficient in the absence of a way to guide the search to promising areas of the large search space. To address this issue, we 
take inspiration from \cite{pairet2021} and
utilize trajectory biasing, and seek to rapidly find a path that satisfies the task plan. We propose to do this by using a simplified motion model of the system and include approximate belief dynamics (\sbd). By simplifying the dynamics of the system while still retaining some belief information, we are able to obtain a calculated trade-off between speed of finding a simplified solution path for guidance and informative guides in the belief space. Below, we formalize this idea for \sbd.

First, we create a lower dimensional state space $\tilde{X}$ which is a subspace of the state space $X$ based on the projection $\tilde{x} = Proj(x)$ 
% \begin{align}
%     \tilde{x} = Proj(x)
% \end{align}
where $Proj: X \rightarrow \tilde{X}$ maps $x \in X$ to $\tilde{x} \in \tilde{X}$. This simplified state space can be arbitrarily chosen, with the only condition being that the new subspace $\tilde{X}$ contains the subspace of all the polytopic regions $\mathcal{P}$, i.e., $p_i \subseteq \tilde{X}$ $\forall p_i \in \mathcal{P}$. If the polytopic regions require all dimensions of the state space, \sbd can still be used, albeit with $\tilde{x} = x$. 
% However, in many applications, the polytopic regions of interest are in subsets of the state space.

Second, we design a simplified motion model and measurement model for $\tilde{x}$. These models can also be arbritrarily chosen, but a general rule is to have simpler models for $\tilde{x}$ than $x$, since the purpose of \sbd is to compute approximate solutions rapidly in order to guide the belief search layer. Some generally applicable examples of simplified models are those with simple first order dynamics and kinematic models. One could also use simplifications such as: (i) geometric planning that ignores uncertainty, (ii) using System~\eqref{eq:system} and ignoring process and measurement noise, and (iii) using System~\eqref{eq:system} and ignoring measurement noise.

% \qh{Is this paragraph too vague?}\zs{Is there a way to describe the relationship between the $x$ dynamics and the $\tilde{x}$ dynamics? If it can be chosen arbitrarily, why shouldn't I choose SR-71 dynamics to approximate a Prius? Maybe there is not a mathematically precise notion, but the description might be improved with even an imprecise notion.}

% \qh{TODO: General rules for augmented motion model and measurement models; 1st order kinematics? Can reduce it further by choosing maximum velocity... This is usually chosen by the user or based on system constraints.}. % This idea of \sbd is general and can be used for general robotics applications, but we focus our attention on the following. 

For many robotic LTL tasks, the regions of interest are defined in the workspace. Therefore, we seek to design a motion model that generates simple kinematic trajectories. To do this, we take advantage of the observation that geometric paths can be interpreted as kinematic trajectories with a fixed speed in each direction. Thus, 
% we compute the maximum speed $v_{max}$ of the robot, based on system constraints 
we use the maximum speed $v_{max}$ of the robot. For the $i$th component of state $\tilde{x}$ denoted by $\tilde{x}_{k}^{(i)}$, the motion model becomes:
\begin{align}
    \tilde{x}_{k+1}^{(i)} = \tilde{x}_{k}^{(i)} + v_{i},
\end{align}
such that $\sum v_{i}^2 = v_{max}^2$. As a simple approximation, we maintain the covariance of the original system using the equations in \eqref{sec:beliefpropagationandlabel}. We refer to this \sbd as Simple Belief Approximated-\sbd (SBA-\sbd).

% In this work, we demonstrate the generality/simplicity/applicability of this idea by considering the following example.

% \ml{define the general rules for the simplified model... 1st order kinematics? Can reduce it further by choosing maximum velocity...}\qh{This is what the example was supposed to be for}
% \qh{TODO: Some segue sentences into analyzing what makes a good \sbd}

% \ml{use words in the assumptions to clarify the intuition}
% \qh{TODO, Maybe?: Need to update assumptions based on $\tilde{\pi^{\alpha}}$.}

% \qh{I put two definitions for admissible here, which one sounds better?}
% \ml{how about Def. 5?}
% \begin{definition}[Admissible \sbd]
%     Consider the projection from $X$ to the projected space $\tilde{X}$ for a \sbd. The \sbd is admissible if there always exists a solution using \sbd in $\tilde{X}$ for every problem instance that a solution to Problem~\ref{prob:1} with the original system exists.
% \end{definition}

% \begin{definition}[Admissible \sbd]
%     Consider the projection from $X$ to the projected space $\tilde{X}$ for a \sbd. The \sbd is admissible if for all instances of Problem~\ref{prob:1}, the existence of a solution for the original system implies that a solution exists for \sbd in $\tilde{X}$.
% \end{definition}

\begin{definition}[Admissible \sbd]
    Consider System \eqref{eq:system} with $X$ and its subspace $\tilde{X}$ for a \sbd. The \sbd is admissible if, for every instance of Problem~\ref{prob:1} that admits a solution for System \eqref{eq:system}, a solution also exists for the \sbd in $\tilde{X}$.
\end{definition}


% \qh{TODO by Saturday: Projection of motion plan full dimensional system. If there exists a motion plan for that system, reduced order model will find it in reduced space (because of covariance lower, or collision lower, or $\pi$...)}

% \begin{lemma}[Admissible \sbd]
    % Suppose a feasible solution to a \sbd exists. Then, a feasible solution to Problem~\ref{prob:1} exists if the \sbd is admissible.
% \end{lemma}
% \begin{proof}[Proof Sketch]
%     Use assumptions \ref{as:covariance decrease phi better} and \ref{as: covariance decrease CC better}.
% \end{proof}

Since the purpose of \sbd is to find a solution quickly to guide the belief search layer, it is desirable to use admissible \sbds. However, the algorithm can still be probabilistically complete if the \sbd is not admissible, as we discuss in Sec.~\ref{sec:analysis}.

In many robotics scenarios, low robot uncertainty is more desirable than high uncertainty. The intuition is that large uncertainty leads to higher risks (e.g., collision probability). However, mathematically, when bad regions (e.g., obstacles) are small, large uncertainty can reduce risk. To rule out such unintuitive cases, we make the following assumption, which we also use to build our \sbd methodology.

\begin{assumption}
    \label{as:covariance decrease phi better}
    If $b_a = \mathcal{N}(\check{x}, \Sigma_a)$, $b_b = \mathcal{N}(\check{x}, \Sigma_b)$, and $\Sigma_a < \Sigma_b$, then 
    \begin{itemize}
        \item For $\alpha < 0.5$: $\pi^{\alpha} \in L(b_b) \implies \pi^{\alpha} \in L(b_a)$.
        \item For $\alpha > 0.5$: $\pi^{\alpha} \notin L(b_b) \implies \pi^{\alpha} \notin L(b_a)$
    \end{itemize}
\end{assumption}

Assumption \ref{as:covariance decrease phi better} states that increasing the covariance does not increase the probability of being in a region at a given state mean for low $\alpha$, which corresponds to `reach' regions. Additionally, increasing the covariance does not increase the probability of not being in a region at a given state mean for high $\alpha$, which corresponds to `avoid' regions. 
% These assumptions may be violated for problems with very small regions and systems with high covariances, but is reasonable for many problems in robotics since we do not generally want to increase uncertainty in order to satisfy chance constraints. This assumption is not required for the correctness of our proposed framework, but we use this intuition to build our \sbd guiding methodology.

\begin{lemma}
    SBA-\sbd is admissible under Assumption \ref{as:covariance decrease phi better}.
\end{lemma}
\begin{proof}[Proof Sketch]
    Starting from the same $\tilde{x}_0$ and the same covariance, SBA-\sbd is able to under-approximate the uncertainty of the belief of the original system at any $\tilde{x}$, since it is a less constrained model. Using Assumptions~\ref{as:covariance decrease phi better}, a lower covariance at each state leads to better probability of satisfaction. There exists at least as many accepting belief trajectories for \sbd as for the full system.
\end{proof}
Finally, the goal is to find a feasible solution for the \sbd augmented version of Problem~\ref{prob:1} in each iteration of the planning framework. Using the hybrid search tree in
Sec.~\ref{sec:gbt}, we obtain a kinematic trajectory for the simplified space $\tilde{X}$. A \sbd path is then the hybrid path $\xi_{\tilde{X}} = (\mathbf{\tilde{x}}, \mathbf{q})$ which is a sequence of pairs of $\tilde{x}$ and $\automaton$ state $q$.

\subsection{Belief Search Layer}
\label{sec:fullplanning}
To guide the search for a solution for the original constrained System~\eqref{eq:system}, we lift \sbd path $\xi_{\tilde{X}}$,  from $\tilde{X}$ to $X$ and use biased sampling around the lifted trajectory set.
% a lifting operator $Lift : \xi_{\tilde{X}} \rightarrow \xi_{X}$ is used 

% We leverage results from \cite{pairet2021}, which shows that biasing sampling around a previously computed kinematic trajectory enables finding solutions faster while maintaining probabilistic completeness. Different from their method which biases search based on a continuous trajectory for single goal planning, a \sbd path is a hybrid trajectory of both kinematic states $\tilde{x}$ and automaton states $q$. Biasing search naively by disregarding automaton states is counter-productive, as many segments of a \sbd path are irrelevant for a tree node with any given automaton states, especially for problems with more complex specifications.

% We leverage results from \cite{pairet2021}, which shows that biasing sampling around a previously computed kinematic trajectory enables finding solutions faster while maintaining probabilistic completeness. Different from their method which biases search based on a continuous trajectory for single goal planning, a \sbd path is a hybrid trajectory of both kinematic states $\tilde{x}$ and automaton states $q$. Biasing search naively by disregarding automaton states is counter-productive, as many segments of a \sbd path are irrelevant for a tree node with any given automaton states, especially for problems with more complex specifications.

% \qh{Unclear how you can sample good controls from
% a reference low dim SiMBA trajectories,}

We propose to bias the belief tree search by using only the \textit{sub-task relevant} segments of $\xi_{\tilde{X}}$.
Let $\text{v}$ be an existing tree node in the belief search layer with discrete component $\text{v}.q_i$, and let $q_{i+1}$ be the successor of $q_i$ in task plan $\mathbf{T}$.
% , which refers to the parts of the \sbd path which directly helps a tree node complete its sub-task (reach a successor state in task plan $\mathbf{T}$). 
% Specifically, 
% for an existing tree $v$ node with discrete component $v.q_i$, we evaluate the successor of $q$  $q_{i+1}$ in $\mathbf{T}$, 
Then, we use the segment of $\xi_{\tilde{X}}$ with discrete components $q_i$ and those that lead to a transition from $q_i$ to $q_{i+1}$, 
i.e., the segment is of the form $\xi^{q_i}_{\tilde{X}} = (\tilde{x}_k, q_i)...(\tilde{x}_{k+m}, q_i)(\tilde{x}_{k+m+1}, q_{i+1})$, where $k$ is the first time step $\xi_{\tilde{X}}$ encounters $q_i$ and $m \geq 0$.
% i.e., $\xi^{q_i}_{\tilde{X}} = \{(\mathbf{\tilde{x}}, \mathbf{q}) \in \xi \mid q = q_i \vee q^- = q_i\}\}$ where $q^{-}$ refers to the predecessor of $q$. 
% The lifting operator is then $Lift(\xi^{q_i}_{\tilde{X}} )$, and 
The sampling bias technique is as follows: given a starting radius $d$ which is incrementally increased, samples are chosen within $d$ radius of $\xi^{q_i}_{\tilde{X}}$ with probability $pr$, and uniformly in the belief space with probability $1-pr$.

% given a starting radius $d$, the planner adjusts $d$ within a range of a strictly guided sampling to a uniform search with $p$ probability, and uniformly over the space with probability $1-p$.

At each iteration, the two layers, \sbd guide and belief search, are given a user-defined time bound to extend the belief tree. The intuition is to continually feedback feasibility information from the tree search layers to the task planning layer. Weights on $\automaton$ are updated based on \eqref{eq:automatonweights} and the algorithm continues to the next iteration.

==> sections/Notes.tex <==
We can use ideas from Belief Roadmap... Herbert's Fasttrack (simplified dynamics). In essence, this method is vaguely similar to FastTrack, planning fast and slow, where our 'fast' planner is one with simplified belief dynamics that provides the lead path to guide the 'slow' planner with full belief dynamics.

We also want to show that even with a suboptimal ROM, we can improve the solution just by virtue of lead guides having some sort of belief information. Lead is like rollout in POMDP planning. A suboptimal solution is obtained via a rollout approach, which is a prominent class of reinforcement learning (RL) methods based on approximation in value space.

\begin{enumerate}
    \item Take only subset of state space that has position. Effectively means that non-position states are fully observable.
    \item Use same Q and R values for the subset of states...
\end{enumerate}

Analysis ideas:

We want to prove that this reduced-order method is an optimistic planner for the true system, i.e. if there exists a solution for the true system, there will always exist a solution for the reduced-order system.

If A matrix is always greater than 1 (diagonal terms, or eigenvalues), then $APA^T + Q$ is always increasing...

ROM covariance grows slower than true model?

keep same measurement regions and measurements.

==> sections/Problem.tex <==
\section{Problem Formulation}
\label{sec:problemstatement}


Consider a robot with both motion and sensing uncertainty tasked with a complex navigation task in a bounded workspace $W \subset \reals^d, d \in \{2, 3\}$. We are interested in computing a motion plan for the robot to achieve its task with robustness guarantees. Below, we formalize this problem.

% \ml{do you need this sentence? you repeat it right after Eq. (2)!}
% Let $\mathcal{X} \subset \reals^n$ and $\mathcal{U} \subset \reals^m$ be the state and control spaces, respectively. Then, t

The robot has linear or linearizable motion and measurement models given by:
\begin{equation}
    \label{eq:system}
    \begin{split}
        &x_{k+1} = Ax_{k} + Bu_{k} + \omega_k, \;\omega_k \sim \N(0, \mathcal{Q}),\\
        &z_k = Cx_k + Du_{k} + \nu_k(x_k),  \;\nu_k(x_k) \sim \N(0, \mathcal{R}(x_k)),
    \end{split}
\end{equation}
where $x_k \in X \subset \reals^n$ is the state, $u_k \in U \subset \reals^m$ is the input, and $z_k \in \reals^p$ is the measurement. Furthermore, matrices $A \in \reals^{n\times n}$, $B \in \reals^{n\times m}$, and $C \in \reals^{n\times p}$. Noise terms $\omega_k$ and $\nu_k$ are i.i.d. random variables with zero-mean Gaussian distributions and covariance matrices $\mathcal{Q}$ and $\mathcal{R}(x_k)$, respectively. Note that covariance $\mathcal{R}(x_k)$ depends on state $x_k$, i.e., it is state-varying measurement noise. This describes problems common in robotics where measurements may be available only in parts of the environment or measurement quality is affected by the state of the robot.
% \ml{could discuss that the linear dynamics could be obtained by feedback linearization or learning from data...}
% We assume that the robot dynamics is linear or linearizable, \qh{papers that it can be linearized, or learnt from data... etc (Vijay Kumar's paper)}

The evolution of the robotic system in \eqref{eq:system} can be described by a discrete-time Gauss-Markov process \cite{gaussmarkovprocess}. The robot state $x_k$ at each time step is a random variable with a Gaussian distribution, i.e., $x_k \sim b_k = \N(\xhat_k, \cov)$, where $b_k \in \B$ is referred to as the \textit{belief} of the robot state, $\B$ is the \textit{belief space}, and $\xhat_k$ and $\cov$ are the state mean and covariance matrix, respectively. A \textit{belief trajectory} $\pb = b_0b_1b_2\cdots b_f$ is a sequence of beliefs.

% \begin{assumption}[Unsatisfiable Specification]
%     A specification is not satisfiable by any belief trajectory for System~\ref{eq:system} if 
% \end{assumption}


\subsection{Linear Temporal Logic over Finite Traces for Belief Tasks} %\ml{what are belief models? Belief Tasks?  Or Task Description in Belief Space?}

The robot is tasked with a temporal specification over the belief space, similar to \cite{Sadigh2016RSS, haesaert2018, Silva2021, CCTL2018, perceptionuncertaintyLTL}.
Let $\mathcal{P} = \{p_1, \cdots, p_n\}$ be a set of convex
polytopic regions in the state space $X$, i.e., $p_i \subset X$ for all $1 \leq i \leq n$.
Further, let $\alpha_i \in [0,1]$ be a probability threshold (chance constraint) on $p_i$.  Then, we define atomic proposition $\pi_i^{\alpha_i}$ associated with region $p_i$ as follows: $\pi_i^{\alpha_i}$ is true for belief $b_k$ iff $P(x_k \in p_i) > 1 - \alpha_i$. This definition states that a proposition is true if the probability that a belief state is in a region $p_i$ is at least $1 - \alpha_i$.
Hence, the set of atomic propositions is $\Pi = \{\pi^{\alpha_i}_i \mid i = 1, \cdots, n\}$.  
% It defines an \textit{alphabet} $AP := 2^{\Pi}$ where each \textit{letter} $\sigma$ of the alphabet is a subset of $\Pi$. 
% A finite string of letters is a finite word $\word = \sigma_1\sigma_2\cdots \sigma_n$ where $\sigma \in AP$. 
% A labelling function $L : B \rightarrow AP$ maps belief states to letters in the alphabet, such that a belief trajectory generates a word with respect to which system properties can be expressed.

We define a labeling function $L : \B \rightarrow 2^\Pi$ that maps a belief $b \in \B$ to the set atomic propositions in $\Pi$ that are true for $b$. 
Then, a belief trajectory $\pb = b_0\cdots b_f$ generates an observation trace (word) $\word = \word_0 \cdots \word_f$ via the labeling function such that $\word_i = L(b_i)$ for all $0 \leq i \leq f$.  Each $\word_i \in 2^\Pi$ is called a symbol.

% \footnote{Note that our approach is not limited to LTLf. Any temporal logic over finite trajectories that can be converted into a finite automaton, such as Metric Interval Temporal Logic \cite{lars, alur}, STL \cite{AGTCDC2022}, can also be used in a similar manner.
% \ml{hmm... big claim here! Need to support this claim... Are you sure nobody can argue against it? think about predicate vs AP and dense time vs discrete time?}
% }.
% We define the labelling function as follows:
% \begin{align}
%     \label{eq:probabilistic_proposition}
%     \pi_i^{\alpha_i} \in L(b_k) \iff P(x_k \in p_i) > 1 - \alpha_i
% \end{align}

% Then, let $\Pi = \{\pi^{\alpha_i}_i|i = 1, \cdots, n\}$ be a set of atomic propositions that is parameterized with a confidence threshold $\alpha_i$. It defines an \textit{alphabet} $AP := 2^{\Pi}$ where each \textit{letter} $\sigma$ of the alphabet is a subset of $\Pi$. A finite string of letters is a finite word $\word = \pi^{\alpha_1}_1\pi^{\alpha_2}_2\cdots \pi^{\alpha_n}_n$ where $\pi^\alpha \in AP$. A labelling function $L : B \rightarrow AP$ maps belief states to letters in the alphabet, such that a belief trajectory generates a word with respect to which system properties can be expressed. We define the labelling function as follows:
% \begin{align}
%     \label{eq:probabilistic_proposition}
%     \pi_i^{\alpha_i} \in L(b_k) \iff P(x_k \in p_i) > 1 - \alpha_i
% \end{align}
% \ml{it would be easier to read if we define the atomic propositions earlier (see comment above). Then the syntax of LTLf becomes very intuitive. Right now the definition of atomic proposition is a little twisted.}

% This labelling function denotes that a proposition is true if the probability that a belief state is within a region is at least $1 - \alpha$.
\begin{definition}[LTLf Syntax \cite{ltlf}]
 Let $\Pi$ be a set of atomic propositions. Then, an LTLf formula over $\Pi$ is recursively defined by:
    \begin{align*}
        \phi := \pi^\alpha \mid \neg \phi \mid \phi \vee \phi \mid \tempop{X} \phi \mid \phi \until \phi
    \end{align*}
where $\pi^\alpha \in \Pi$ is an atomic proposition, $\neg$ (``negation'') and $\vee$ (``or'') are Boolean operators, and  $\tempop{X}$ (``next'') and $\until$ (``until'') are the temporal operators.
\end{definition}

\noindent From this definition, one can derive other standard temporal operators, e.g., the $\eventually$ ("eventually") and $\globally$ ("globally") operators are given by $\eventually \phi \equiv \top \until \phi$ and $\globally \phi \equiv \neg \eventually \neg \phi$.

LTLf formulas are interpreted over finite words in $(2^{\Pi})^*$. The semantics of LTLf can be found in \cite{ltlf}. We say a finite trace $\sigma$ satisfies formula $\phi$, denoted by $\sigma \models \phi$, iff $\sigma, 0 \models \phi$. 
Additionally, we say that a belief trajectory satisfies a specification $\phi$, written $\mathbf{b} \models \phi$, if its generated word $\word = L(b_0)L(b_1)\cdots L(b_n)$ satisfies $\phi$, i.e., $\word \models \phi$.
% \begin{definition}[LTLf Semantics \cite{ltlf}]
% Given a finite word $\word \in (2^\Pi)^*$, denote by $|\word|$ and $\word_i$ the length of $\word$ and the symbol in the $i^{th}$ position in $\word$, respectively.  Then, the satisfaction of an LTLf formula by word $\word$ at time step $i$ is recursively defined by
% \begin{itemize}
%     \item $\sigma, i \models \top$; 
%     \item $\sigma, i \models \pi^{\alpha} \iff \pi^{\alpha} \in \sigma_i$;
%     \item $\sigma, i \models \neg \pi^{\alpha} \iff \sigma, i \not\models \pi^{\alpha}$;
%     \item $\sigma, i \models \phi_1 \vee \phi_2 \iff \sigma, i \models \phi_1 \vee \sigma, i \models \phi_2$;
%     % \item $\sigma, i \models \phi_1 \vee \phi_2 \iff \sigma \models \phi_1 \vee \sigma \models \phi_2$;
%     \item $\sigma, i \models \tempop{X}\phi \iff \sigma, i+1 \models \phi$;
%     \item $\sigma, i \models \phi_1 \until \phi_2 \iff \exists j \in \mathbb{N},\; i \leq j \leq |\sigma|$, s.t. $\sigma, j \models \phi_2 \text{ and } \forall k, i \leq k < j, \text{ we have } \sigma, k \models \phi_1$.
% \end{itemize}

% \end{definition}

% \noindent We say a finite trace $\sigma$ satisfies formula $\phi$, denoted by $\sigma \models \phi$, iff $\sigma, 0 \models \phi$. 
% Additionally, we say that a belief trajectory satisfies a specification $\phi$, written $\mathbf{b} \models \phi$, if its generated word $\word = L(b_0)L(b_1)\cdots L(b_n)$ satisfies $\phi$, i.e., $\word \models \phi$.

% Note that the negation of an atomic proposition $\neg \pi^{\alpha}$ means the probability of visiting region $r$ must be at least $1 - \alpha$, i.e., $\neg \pi^{\alpha} \equiv \neg \Big( P(x_k \in p_i) > 1 - \alpha \Big) \equiv \Big( P(x_k \in p_i) \leq 1 - \alpha \Big)$.  For small $\alpha$, . In my applications, one might be interested in avoiding the region $p_i$ with high probability. Similar to \cite{Nathalie2019}, we can do this by capturing the more intuitive converse of $\pi^{\alpha}_{i}$ by adding new atomic propositions. This can be done by associating to each $p_{i}$ a new atomic proposition $\tilde{\pi}^{\alpha}_{i}$ that is true for belief $b_k$ iff $P(x_k \notin p_i) \geq 1 - \alpha$, such that $\tilde{\pi}^{\alpha}_{i}$ represents $\neg {\pi}^{1 - \alpha}_{i}$.

% \ml{this paragraph is hard to parse... I think what you're trying to say is that if we want to be in a region with a high probability (small alpha) for some part of the formula and then avoid the same region with a high probability in another part of the formula, then the same alpha wouldn't work.  Is that right?  If so, then say it that way.}\qh{You could also want to be in a region with low probability for some reason}\qh{But yes}\ml{If the atomic proposition is used only once, then you can use a large alpha to avoid the region, no?}\qh{True. Does this make more sense now? Technically, we don't really need to add this new set of atomic propositions, because we can just have different atomic propositions for different $\alpha$, right? This is just for convenience}\ml{Absolutely... we can say either define multiple alphas for the same $p$ or extend $\Pi$ by $1-\alpha$ propositions, which is essentially the same approach.}
% \ml{proofread this:}
Note that, for a small $\alpha$, $\pi_i^\alpha$ requires being in region $p_i$ with a high probability.  
The negation of it, $\neg \pi^{\alpha} = P(x_k \in p_i) \leq 1 - \alpha$, still allows being in region $p_i$ with a relatively high probability. In many applications, however, one may be interested in expressing a task for being in a region with high probability in one part of a formula and then avoiding the same region also with high probability in another part of the formula. Similar to \cite{Nathalie2019}, we can do this by capturing the more intuitive converse of $\pi^{\alpha}_{i}$ by adding new atomic propositions. This can be done by associating to each $p_{i}$ a new atomic proposition $\tilde{\pi}^{\alpha}_{i}$ that is true for belief $b_k$ iff $P(x_k \notin p_i) \geq 1 - \alpha$, such that $\tilde{\pi}^{\alpha}_{i}$ represents $\neg {\pi}^{1 - \alpha}_{i}$.

\subsection{Planning Problem}
\label{sec:belief_propagation_equations}

% \ml{hmmm... This subsection could be the problem. No need for equations (7)-(11). After defining (6), you can define the problem.}

We seek a motion plan that satisfies a given LTLf formula $\phi$. 
% \ml{such a convoluted sentence!}
% The motion plan is characterized by a sequence of nominal control inputs and its corresponding nominal state trajectory such that they produce in the absence of uncertainty, along with a linear feedback controller that seeks to follow this trajectory using online state estimate $\xhat_k$.
Assuming that the robot is equipped with a feedback trajectory-following controller,
a motion plan can then be characterized as a sequence of control inputs coupled with its corresponding nominal state trajectory.
Let $\checkU^{0,t} = (\checku_0, \checku_1, \ldots, \checku_{t-1})$ be a sequence of control inputs. Then, given an 
initial belief $b_0$, a nominal trajectory
$\checkX^{x_0,x_t} = (\checkx_0, \checkx_1, \ldots, \checkx_t)$ is obtained by applying $\checkU^{0,t}$
to the nominal system dynamics $\checkx_{k+1} = A\checkx_{k} + B\checku_k$. This motion plan $(\checkU^{0,t}, \checkX^{x_0,x_t})$ is then executed online, given online state estimates $\xhat_k$, via the stabilizing, trajectory-following controller
\begin{align}
    \label{eq:feedback controller}
    u_k = \check{u}_{k-1} - K (\xhat_k - \checkx_k),
\end{align}
where $K$ is the feedback control gain. 
% We refer to $(\checkU,\checkX)$ as a \textit{motion plan} for System \eqref{eq:system}.

% \qh{The belief trajectory $\pb$ that satisfies the specification is what we are after.}
% Now, given a stabilizing feedback controller in \eqref{eq:feedback controller} and online state estimate $\xhat_k$, the system closed-loop dynamics are
% \begin{align}
%     x_k = Ax_k + B\check{u}_{k-1} - K (\xhat_k - \checkx_k) + w_k\text{.}
% \end{align}

% \subsection{LTLf Planning Problem}

% The formal statement of the problem is as follows:

\begin{problem}
    \label{prob:1}
    Given System \eqref{eq:system}, a set of probabilistic atomic propositions $\Prop = \{\prop^{\alpha_1}_1, \ldots, \prop^{\alpha_n}_n\}$ defined over regions $\mathcal{P}$, LTLf formula $\phi$ defined over $\Prop$, and closed-loop control gain K, find a motion plan $(\checkU, \checkX)$ as a pair of sequence of nominal controls $\checkU = (\checku_0,\ldots,\checku_{k-1})$ for some $k\geq 1$ and its resulting nominal trajectory $\checkX = (\checkx_0,\ldots, \checkx_k)$ such that when executed via the controller in \eqref{eq:feedback controller} the resulting belief trajectory $\pb$ satisfies the LTLf formula, i.e., $\pb \models \phi.$
\end{problem}

% \qh{keep in mind the closed loop dynamics vs execution}

% \ml{should talk about the challenges of this problem and how our approach addresses them}

The main challenge in this problem is that the search space is extremely large. This is because planning must be performed in the composition of the belief space with the task space (representation of the set of all satisfying words). For an $n$-dimensional state space, the Gaussian belief space adds $O(n^2)$ dimensions, and for a task formula of size $|\phi|$, the size of the task can be as large as $2^{2^{|\phi|}}$ \cite{ltlf}. Hence, to make the problem computationally tractable, the search must be performed with informed guidance. Existing methods for guiding search in the state space through, e.g., discrete abstractions or geometric planning, fail to capture belief information, leading to uninformative guides. 
To address these challenges, we aim to design a framework that reduces dependence on fine, discrete abstractions, while efficiently searching in the belief space. Specifically, we seek to generate informed guidance via simplified models.
% By leveraging recent advances in Gaussian belief space planning using sampling-based tree search...


% \begin{problem}
%     \label{prob:1}
%     Given System \eqref{eq:system}, a set of probabilistic atomic propositions $\Prop = \{\prop^{\alpha_1}_1, \ldots, \prop^{\alpha_n}_n\}$, a LTLf formula $\phi$ defined over $\Prop$, and a Lipschitz continuous and monotonic cost function $J: \X \to \reals^+$, find a motion plan $(\checkU, \checkX)^*$ as a pair of sequence of nominal controls $\checkU = (\checku_0,\ldots,\checku_{k-1})$ for some $T\geq 1$ and its resulting nominal trajectory $\checkX = (\checkx_0,\ldots, \checkx_k)$ that minimizes the expected total cost, 
%     \begin{equation}
%         (\checkU, \checkX)^* = \arg\min_{(\checkU, \checkX)}\; \mathbb{E} \Big[ \sum_{k=0}^{T} J(x_{k}) \Big],
%     \end{equation}
%     subject to, when executed via controller in \eqref{eq:feedback controller} the resulting belief trajectory $\pb$ \qh{check wording} satisfies the LTLf formula, i.e.
%     \begin{equation}
%         \pb \models \phi.
%     \end{equation}
% \end{problem}

==> sections/Relatedwork.tex <==
\section{Related Work}

Silva et. al (Active Perception and Control from PrSTL Specifications)... counterexample-guided synthesis... maximum likelihood

Pairet's geometric guide

Syclops

Vasile et al, Control in Belief Space with Temporal Logic Specifications - MDP, FIRM with Rabin automaton. Need to explain why we are better than FIRM. Needs to go to steady state kalman filter.

Active Perception and Control from PrSTL Specifications - maximum likelihood assumption, BMC counter-example guided synthesis, abstraction too much?? approach, cannot optimize for cost function, does it actually find feasible trajectories for sure?

Goal POMDPs - assume feasible at all states (goal is reachable from all states).

Abstraction-free approach - assumes geometric is enough.

Sub-goals, abstraction.

Something something dual control objective



==> sections/intro_figure.tex <==
\begin{figure}[t!]
    \centering
    \begin{adjustbox}{scale=0.75}
    \centering
    \begin{tikzpicture}[shorten >=1pt,node distance=6cm,>=stealth',thick, auto,
                        every state/.style={fill,very thick,black!20,text=black,\shadowString},
                        robot/.style = {fill,very thick,black!20,rounded corners, text=black, shape=rectangle, minimum height=1cm,minimum width=1cm, blur shadow},
                        accepting/.style ={blue!50!black!50,text=white,accepting by double},
                        initial/.style ={red!80!black!40,text=black,initial by arrow, initial left}, initial text=$ $]
        \definecolor{color1}{HTML}{E7AD00}
        \definecolor{color2}{HTML}{A5CC19}
        \definecolor{color3}{HTML}{33B29A}
        \definecolor{color4}{HTML}{3380FF}
        \definecolor{color5}{HTML}{9033FF}
        \definecolor{color6}{HTML}{E5003D}
        
        \begin{scope}[
            opacity = 1,
            fill opacity = 0.25,
            text opacity = 1,
            text width = 6em,
            text centered]
            
            % \def\firstrectangle{rectangle (2,4)}
            \def\secondrectangle{(2:4cm) rectangle (2,4)}
            \def\thirdrectangle{(8:4cm) rectangle (2,4)}
            \draw [fill = color6] \firstrectangle;
            \draw [fill = color4] \secondrectangle;
            \draw [fill = color2] \thirdrectangle;
        \end{scope}
        
        % \begin{scope}[minimum width = 1em, text width = 7.0em, text centered, 
        %              every node/.style={font = \footnotesize}     ]

        %     \node (FM) at ( 90:3.5) {\emph{Formal Methods}};
        %     \node (GT) at (210:2.5) {\emph{Game Theory}};
        %     \node (HRI) at (-30:3.0) {\emph{Human Robot Interaction}};
            
        %     \node[font=\scriptsize] (gt_des) [below=0.5em of GT] {Controller Synthesis};
        %     \node[font=\scriptsize] (fm_des) [below=0.5em of FM] {Task Completion Guarantees};
        % \end{scope}
    
    \end{tikzpicture}
    \end{adjustbox}
\caption{3 $\times$ 3 Example WTS}
\label{fig: gridword_ex}
\vspace{-0.5 cm}
\end{figure}
